Analysis of the spatial and dynamical properties of a multiscale model of intestinal crypts

The preliminary analyses on a multiscale model of intestinal crypt dynamics are here presented. The model combines a morphological model, based on the Cellular Potts Model (CPM), and a gene regulatory network model, based on Noisy Random Boolean Networks (NRBNs). Simulations suggest that the stochastic differentiation process is itself sufficient to ensure the general homeostasis in the asymptotic states, as proven by several measures.

==> eptcsdata.tex <==
\providecommand{\firstpage}{79}
\providecommand{\publicationstatus}{A. Graudenzi, G. Caravagna, G. Mauri, M. Antoniotti (Eds.): \\Wivace 2013 - Italian Workshop on \\Artificial Life and Evolutionary Computation\\
EPTCS 130, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.130.12}{10.4204/EPTCS.130.12}}
\pdfoutput=1

